Using Artificial Intelligence to Unlock Crowdfunding Success for Small Businesses

While small businesses are increasingly turning to online crowdfunding platforms for essential funding, over 40% of these campaigns may fail to raise any money, especially those from low socio-economic areas. We utilize the latest advancements in AI technology to identify crucial factors that influence the success of crowdfunding campaigns and to improve their fundraising outcomes by strategically optimizing these factors. Our best-performing machine learning model accurately predicts the fundraising outcomes of 81.0% of campaigns, primarily based on their textual descriptions. Interpreting the machine learning model allows us to provide actionable suggestions on improving the textual description before launching a campaign. We demonstrate that by augmenting just three aspects of the narrative using a large language model, a campaign becomes more preferable to 83% human evaluators, and its likelihood of securing financial support increases by 11.9%. Our research uncovers the effective strategies for crafting descriptions for small business fundraising campaigns and opens up a new realm in integrating large language models into crowdfunding methodologies.

==> sections/method-old.tex <==
\section{Predictive Analysis}


%Dataset
In this study, we collected all fundraising campaigns that fall into the small-business-relief collection of GoFundMe, the largest crowdfunding platform in the world \cite{usnews_2023}, during the most recent pandemic shock from January $22^{nd}$, 2020 to December $31^{st}$, 2020. After excluding campaigns not indeed aimed at supporting individual small businesses, our final dataset comprises 11,274 campaigns, encompassing a diverse range across 50 States.

On GoFundMe, fundraisers seek donations from the general public by posting a fundraising campaign that specifies the fundraising goal amount, relevant photo(s), and a short textual description. To identify the key factors that contribute to fundraising success, we combine behavioral theories and natural language processing tools to construct four groups of features: textual description, campaign meta-setup, demographics in the business local area, and other contextual features. 

%Features
\emph{Textual description}. The campaign description serves as the primary medium for conveying essential information about the fundraising campaign \cite{zhou2018project}. It addresses critical questions such as the reasons a small business asking for the specified financial support, the nature of the small business's services, and the mutual benefits for both the business and its donors. 

However, even with the help of machine learning and natural language processing techniques, it has been traditionally challenging to extract textual features directly related to the fundraising context from such large-scale open-ended and unstructured textual data: Supervised machine learning models require highly-skilled human annotators to get consistent labels for model training,  which is very expensive. Unsupervised models (such as probabilistic topic modeling) can hardly identify meaningful features that are connected to the literature. 

%To approach these questions, we innovatively incorporate the large language model, GPT-4, since the 
Recent advances in large language models (LLM), provide unprecedented powerful tools to extract the key features embedded in campaign descriptions. Leveraging prior literature in crowdfunding and small business domain context \cite{list2021experimental, frey2004social}, we are able to generate 10 features by GPT,  capturing aspects such as social comparison with peer businesses, plan of funding usage, 
%previous business achievements, extrinsic motivation, 
and %challenges
urgency
highlighted in campaign descriptions. 

% \weic{One missing piece here is why do we need both high-level (GPT-extracted) features as well as low-level (lexicon-based) features.}

In addition to discerning key elements of content that should be included in the campaign description, we also control for the style and sentiment of the campaign descriptions, whose effect on effective messaging has been confirmed in prior literature in crowdfunding % investigate how to effectively deliver such messages. Building upon previous literature in crowdfunding adopting automated text analysis tools 
\cite{markowitz2021predictive, rhue2018emotional, tan2016winning}
%, we incorporate LIWC \cite{boyd2022linguistic}, NRC Emotional Lexicon \cite{mohammad2013crowdsourcing},
% concreteness and dominance rating of words 
and beyond \cite{brysbaert2014concreteness, warriner2013norms,wang2015making}. 
% blacklist of spam words \cite{}
We are able to develop 109 features in total, including emotion measurement, text complexity (such as length and syllables per word), as well as text concreteness and dominance. See Support Information \ref{sec:text} for a complete list of textual features.


\emph{Campaign Meta-Setup}. Apart from details revealed in the  textual description, meta-information of a campaign may also affect the fund-raising success. To maximize the predictive power of the machine learning models, we control for the meta information that is associated with the fundraising success, such as the amount of fundraising goal  \cite{chen2023investigating} and the gender of the organizer \cite{ullah2020gender}.

\emph{Local Demographics}. To control for the potential local socio-economic and demographic impact on small businesses and their fundraising outcomes \cite{igra2021crowdfunding}, we draw information from American Community Survey \cite{united2019american} and compile 46 features to capture local contextual factors such as city income level, business volume, citizen educational level. 

\emph{Level of Pandemic Shock}. This group of features represents the severity of the external shock on small business. Similar to the Covid-19 pandemic, the impact levels of an external shock may vary across different cities and states over time, likely influencing the donation preferences of crowdfunding participants \cite{bartik2020impact, mueller2021impacts}. We therefore additionally develop features to capture the local COVID Statistics, such as number of cases and deaths, to assess the extent of the pandemic's impact.


% model selection and problem set up
Leverage the insights from previous literature that more than 40\% of campaigns received no money at all \cite{igra2021crowdfunding}, we then engage these features to predict the fundraising outcome measured as a binary value indicating whether the small business was able to get any financial support from the crowdfunding campaign on GoFundMe \footnote{We collected campaigns created from the beginning of the Covid pandemic to December $31^{st}$, 2020. The information was updated daily until Feb $5^{th}$, 2021). This should give us an excellent estimate of the fundraising outcome given 93.98\% GoFundMe small-business-relief campaigns that received financial support got their first donation within a month after the campaign was publicly posted.} 
%\cite{zribi2022effects}

Since our goal of predictive analysis is not only to test the predictive power of the features, but more importantly to discover actionable insights that inform the optimal writing of crowdfunding campaigns, we selected the Light Gradient-Boosting Machine (LightGBM) \cite{ke2017lightgbm}, a non-linear tree-based machine learning model of high explanability and computational efficiency. Three baselines are incorporated: a uniform prediction baseline, and a random prediction baseline. We followed the standard practices by dividing the dataset into training, validation, and test sets based on the campaign posting date, as shown in Table \ref{tab:data_split}. We rigorously tune the hyperparameters of the machine learning models based on validation F1-score and report the performance of the models on test set (fundraising campaigns starting in May, 2020) as shown in Table \ref{tab:lgb}.

%\weic{cannot find the table. table in main text and SI should be numbered separately. }



